AiRound and CV-BrCT: Novel Multi-View Datasets for Scene Classification

It is undeniable that aerial/satellite images can provide useful information for a large variety of tasks. But, since these images are always looking from above, some applications can benefit from complementary information provided by other perspective views of the scene, such as ground-level images. Despite a large number of public repositories for both georeferenced photographs and aerial images, there is a lack of benchmark datasets that allow the development of approaches that exploit the benefits and complementarity of aerial/ground imagery. In this paper, we present two new publicly available datasets named \thedataset~and CV-BrCT. The first one contains triplets of images from the same geographic coordinate with different perspectives of view extracted from various places around the world. Each triplet is composed of an aerial RGB image, a ground-level perspective image, and a Sentinel-2 sample. The second dataset contains pairs of aerial and street-level images extracted from southeast Brazil. We design an extensive set of experiments concerning multi-view scene classification, using early and late fusion. Such experiments were conducted to show that image classification can be enhanced using multi-view data.

==> tex/UDA.tex <==
\subsection{Unsupervised Domain Adaptation (UDA)}
\label{sec:UDAs}

In this work, five feature-based UDA approaches were used for the experiments: (i) Transfer Component Analysis~\cite{pan2011domain}; (ii) Joint Distribution Analysis~\cite{long2013transfer}; (iii) Subspace Alignment~\cite{fernando2013unsupervised}; (iv) Geodesic Flow Kernel~\cite{gong2012geodesic}; and (v) CORAL~\cite{sun2016return}.
Those techniques can be divided in three different categories: data-centric, subspace-centric, and hybrid. 
In the following sections, we introduce those categories and detail the properties of each method.

%We introduce each UDA method according to their branch in the next Sections.

% \begin{table}[h!]
% 	\centering
% 	\caption{Summary of Unsupervised Domain Adaptation Methods}
% 	\label{properties}
% 	\tabcolsep=0.075cm
% 	%\scalebox{0.95}
% 	{
% 		\begin{tabular}{llccccc}
% 			\hline
% 			& Approaches & \begin{tabular}[c]{@{}c@{}}Preserve\\ Variance\end{tabular} & \begin{tabular}[c]{@{}c@{}}Marginal\\ Distribution\end{tabular} & \begin{tabular}[c]{@{}c@{}}Conditional\\ Distribution\end{tabular} & \begin{tabular}[c]{@{}c@{}}Reweight\\ Instances\end{tabular} & \begin{tabular}[c]{@{}c@{}}Geometric\\ Structure\end{tabular} \\ \hline
% 			\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Data\\ Centric\end{tabular}} & TCA~\cite{pan2011domain} & \Checkmark & \Checkmark &  &  &  \\
% 			& JDA~\cite{long2013transfer} & \Checkmark & \Checkmark & \Checkmark &  &  \\
% 			& TJM~\cite{long2014transfer} & \Checkmark & \Checkmark &  & \Checkmark &  \\ \hline
% 			\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Subspace\\ Centric\end{tabular}} & SA~\cite{fernando2013unsupervised} & \Checkmark &  &  &  &  \\
% 			& GFK~\cite{gong2012geodesic} & \Checkmark &  &  &  & \Checkmark \\ \hline
% 			\multirow{2}{*}{Hybrid} & CORAL~\cite{sun2016return} & \Checkmark &  &  &  & \Checkmark \\
% 			& JGSA~\cite{zhang2017joint} & \Checkmark & \Checkmark &  & \Checkmark & \Checkmark \\ \hline
% 		\end{tabular}
% 	}
% \end{table}

% \begin{table}[h!]
% 	\centering
% 	\caption{Summary of the evaluated Unsupervised Domain Adaptation (UDA) methods.}
% 	\label{properties}
% 	\tabcolsep=0.075cm
% 	\scalebox{0.85}
% 	{
% 		\begin{tabular}{llcccc}
% 			\hline
% 			& Method & \begin{tabular}[c]{@{}c@{}}Preserve\\ Variance\end{tabular} & \begin{tabular}[c]{@{}c@{}}Marginal\\ Distribution\end{tabular} & \begin{tabular}[c]{@{}c@{}}Conditional\\ Distribution\end{tabular} & %\begin{tabular}[c]{@{}c@{}}Reweight\\ Instances\end{tabular} &
% 			\begin{tabular}[c]{@{}c@{}}Geometric\\ Structure\end{tabular} \\ \hline
% 			\multirow{2.2}{*}{\begin{tabular}[c]{@{}c@{}}Data-\\ centric\end{tabular}} & TCA~\cite{pan2011domain}  & \Checkmark & \Checkmark & &  \\
% 			& JDA~\cite{long2013transfer}  & \Checkmark & \Checkmark & \Checkmark & \\
% 			%& TJM~\cite{long2014transfer}  & \Checkmark &  & \Checkmark &  \\
% 			\hline
% 			\multirow{2.3}{*}{\begin{tabular}[c]{@{}c@{}}Subspace-\\ centric\end{tabular}} & SA~\cite{fernando2013unsupervised}  & \Checkmark &  &  & \\
% 			& GFK~\cite{gong2012geodesic}  & \Checkmark &  &  & \Checkmark \\ \hline
% 			Hybrid & CORAL~\cite{sun2016return}  & \Checkmark &  &  & \Checkmark \\
% 			%& JGSA~\cite{zhang2017joint}  & \Checkmark &  & \Checkmark & \Checkmark \\
% 			\hline
% 		\end{tabular}
% 	}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Data-centric Approaches}

In data-centric methods, there is a premise of the existence of a projection transformation from both domains into another space that is domain-invariant. 
In that way the domain shift between both domains is reduced, without modifying data properties from the original spaces~\cite{pan2011domain,long2013transfer}.
For this group of methods, we evaluated two of them. A description of how the methods that were used work can be found below.

% Original
%To align source and target data, data-centric methods attempt to find a specific transformation that can project both domains into a domain-invariant space.
%The divergence between domains is reduced, while preserving the data properties from the original spaces~\cite{pan2011domain,long2013transfer}.
%Two data-centric UDA approaches were evaluated in this work. 

\noindent \textbf{Transfer Component Analysis (TCA)}~\cite{pan2011domain}.
The main objective of TCA is to learn a set of transfer components that lies in a Reproducing Kernel Hilbert Space. In this way, projecting data into this space spanned by the transfer components, it is possible to reduce the domain shift between source and target domains.

%learn a set of a set of transfer components that lies in a in a Reproducing Kernel Hilbert Space. 
%In this way, when the domain data is projected onto the latent space spanned by the transfer components, the domain shift between different distributions across domains is reduced, while the variance is preserved.

% Original
%\noindent \textbf{Transfer Component Analysis (TCA)}~\cite{pan2011domain}. 
%The goal of this method is to learn a set of transfer components in a Reproducing Kernel Hilbert Space.
%When projecting domain data onto the latent space spanned by the transfer components, the distance between different distributions across domains is reduced and variance is preserved.

\noindent \textbf{Joint Distribution Adaptation (JDA)}~\cite{long2013transfer}. 
An extension of the Maximum Mean Discrepancy (MMD) is created to measure the difference in both marginal and conditional distributions. Even minimizing the marginal distribution between the source and target data, TCA does not ensure that conditional distributions between domains are reduced, which may lead to a poor adaptation. The JDA attempt to improve TCA, integrating MMD jointly with Principal Component Analysis (PCA), creating a robust and effective feature representation for large domain shifts.

% Original
%\noindent \textbf{Joint Distribution Adaptation (JDA)}~\cite{long2013transfer}. 
%This method extends the Maximum Mean Discrepancy (MMD) to measure the difference in both marginal and conditional distributions. Despite minimizing the marginal distribution between the source and target data, TCA does not guarantee that conditional distributions are reduced in this formulation, which may lead to a poor adaptation.
%JDA improves TCA and integrates MMD with Principal Component Analysis (PCA) to create a feature representation that is effective and robust for large domain shifts. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Subspace-Centric Approaches}

The main differences between domain and subspace-centric methods is that subspace-centric methods work with manipulations of subspaces between different domains~\cite{gong2012geodesic}, while domain-centric methods deals with unified transformations. For this subgroup of methods, we evaluated two of them. A description of how the methods that were used work can be found bellow.

%In contrast to data-centric methods, subspace-centric methods do not assume the existence of a unified transformation.
%They rely on a subspace manipulation of the source and target domains~\cite{fernando2013unsupervised} or between them~\cite{gong2012geodesic}, upholding that separate subspaces have very optional particular features to be exploited.
%Two subspace-centric UDA techniques were evaluated in this work. 

\noindent\textbf{Subspace Alignment (SA)}~\cite{fernando2013unsupervised}.
In this method, the Principal Component Analysis algorithm is applied to project the source and target domains on different subspaces. After that, the method can be expressed as an optimization problem where the main objective is to learn a transformation matrix that is used to align both subspaces minimizing the Frobenius norm of their difference.


% \noindent\textbf{Subspace Alignment (SA)}~\cite{fernando2013unsupervised}.
% This approach projects source and target data onto different subspaces using PCA.
% The method then learns a linear transformation matrix that aligns the source subspace to the target one while minimizing the Frobenius norm of their difference.

\noindent \textbf{Geodesic Flow Kernel (GFK)}~\cite{gong2012geodesic}.
% apos keiller
%This technique explores the information of intermediate subspaces between projections of source and target data to learn domain-invariant features. However, instead of using a finite number of subspaces, the method integrates an infinite number of subspaces that lie on the geodesic flow from the source subspace to the target and explicitly construct an infinite-dimensional feature space.
This technique exploits the intermediate subspaces between projections of source and target data to learn domain-invariant features. However, instead of using a finite number of subspaces, the method integrates an infinite number of subspaces that lie on the geodesic flow from the source subspace to the target and explicitly construct an infinite-dimensional feature space.

% Original
%This approach explore the information of intermediate subspaces between projections of source and target data to learn domain-invariant features. However instead of using a finite number of subspaces, the method integrates an infinite number of subspaces that lie on the geodesic flow from the source subspace to the target.



%This technique explores the information of intermediate subspaces between projections of source and target data to learn domain-invariant features. However, instead of using a finite number of subspaces, the method integrates an infinite number of subspaces that lie on the geodesic flow from the source subspace to the target and explicitly construct an infinite-dimensional feature space.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Hybrid Approaches}

Attempting to avoid some of the aforementioned methods disadvantages, hybrid approaches emerges without need to use subspace projections or assume unified transformations.

\noindent\textbf{CORAL}~\cite{sun2016return}.
This algorithm focuses on dealing with the disadvantages of both subgroups, previously mentioned.
The differences between source and target domain are decreased using the alignment of both distributions in the input data.
%minimized by aligning the covariance of the source and target distributions in the original data.
In opposition to the SC methods, this algorithm 
deals with data alignment in a way that a subspace projection is not necessary, and because of that to execute it is necessary high computation resources and complex tuning of hyper-parameters.
Finally, it is important to mention that unlike domain-centric algorithms, CORAL works with asymmetric transformations and it only applies them on source data.


%suggests an alignment without the need for subspace projection, %which would require intense computation and complex hyper-parameter tuning.
%In addition, CORAL~\cite{sun2016return} does not assume a unified transformation like data-centric methods; it uses, instead, an asymmetric transformation only on source data. 


==> tex/acknowledgment.tex <==
% Use section* for acknowledgment
\section*{Acknowledgment}


The authors would like to thank...

==> tex/biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Michael Shell}
Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{John Doe}
Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Jane Doe}
Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
